Of All StrIPEs: Investigating Structure-informed Positional Encoding for Efficient Music Generation

While music remains a challenging domain for generative models like Transformers, a two-pronged approach has recently proved successful: inserting musically-relevant structural information into the positional encoding (PE) module and using kernel approximation techniques based on Random Fourier Features (RFF) to lower the computational cost from quadratic to linear. Yet, it is not clear how such RFF-based efficient PEs compare with those based on rotation matrices, such as Rotary Positional Encoding (RoPE). In this paper, we present a unified framework based on kernel methods to analyze both families of efficient PEs. We use this framework to develop a novel PE method called RoPEPool, capable of extracting causal relationships from temporal sequences. Using RFF-based PEs and rotation-based PEs, we demonstrate how seemingly disparate PEs can be jointly studied by considering the content-context interactions they induce. For empirical validation, we use a symbolic music generation task, namely, melody harmonization. We show that RoPEPool, combined with highly-informative structural priors, outperforms all methods.

==> sections/discussion.tex <==
\section{Discussion}

==> sections/notation_table.tex <==
% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{ll}
% \hline
% Symbol & Meaning \\ \hline \hline
% $x, \mathbf{x}, \mathbf{X}$ & scalars, vectors and matrices, respectively \\
% $\mathbf{Q}$/$\mathbf{K}$  & ``$\mathbf{Q}$ (respectively $\mathbf{K}$)''        \\
%        &        \\ \hline
% \end{tabular}%
% }
% \end{table}

==> sections/proofs/derivations_toy.tex <==
\noindent\textbf{IV. Derivations for toy example} corresponding to Equations (24), (25) and (26).\\

\noindent For RoPE, we can derive the expression as:
\begin{align*}
    a_{mn} \approx & \sum_{d=1}^{D/2} (q_{m,2d-1} k_{n,2d-1} + q_{m,2d} k_{n,2d} )
    \cos \Delta^-_d  + \\ &
    ( q_{m,2d-1} k_{n,2d} - q_{m,2d} k_{n,2d-1} )
    \sin \Delta^-_d\\
    = & 
    \sum_{d=1}^{D/2} \left[ \begin{array}{cc}
     q_{m, 2d-1} & q_{m, 2d}
    \end{array}\right]
    \left[ \begin{array}{c}
     k_{n, 2d-1} \\ k_{n, 2d}
    \end{array}\right]\cos \Delta^-_d + \\ & \left[ \begin{array}{cc}
     q_{m, 2d-1} & q_{m, 2d}
    \end{array}\right]
    \left[ \begin{array}{c}
     k_{n, 2d} \\ - k_{n, 2d-1}
    \end{array}\right]\sin \Delta^-_d\\
    = &
    \sum_{d=1}^{D/2} \left[ \begin{array}{cc}
    \cos \psi_q^d & \sin \psi_q^d
    \end{array}\right]
    \left[ \begin{array}{c}
     \cos \psi_k^d \\ \sin \psi_k^d
    \end{array}\right]\cos \Delta^-_d \\ & + 
    \left[ \begin{array}{cc}
     \cos \psi_q^d & \sin \psi_q^d
    \end{array}\right]
    \left[ \begin{array}{c}
     \sin \psi_k^d \\ - \cos \psi_k^d
    \end{array}\right]\sin \Delta^-_d\\
    = &
    \sum_{d=1}^{D/2} \cos (\psi_q^d - \psi_k^d )\cos \Delta^-_d + \sin (\psi_k^d - \psi_q^d ) \sin \Delta^-_d\\
    = &
    \sum_{d=1}^{D/2} \cos (\psi_q^d - \psi_k^d )\cos \Delta^-_d - \sin (\psi_q^d - \psi_k^d ) \sin \Delta^-_d\\
    = & \sum_{d=1}^{D/2} \cos \big( ( \psi_q^d - \psi_k^d ) + f_d ( \xi_m^d - \xi_n^d ) \big)
\end{align*} 
where $\Delta^-_d = f_d ( \mathcal{P}_Q[m] - \mathcal{P}_K[n] ) = f_d ( \xi_m^d - \xi_n^d )$.

For F-StrIPE$_1$, we can derive the expression as:
\begin{align*}
    a_{mn} \approx & \sum_{d=1}^D q_{md} k_{nd} \cos \Delta^-_d \\
    = & 
    \sum_{d=1}^{2/D} \left[ \begin{array}{cc}
     q_{m, 2d-1} & q_{m, 2d}
    \end{array}\right] \left[ \begin{array}{c}
     k_{n, 2d-1} \\ k_{n, 2d}
    \end{array}\right] \cos \Delta^-_d\\
    = & 
    \sum_{d=1}^{2/D} \left[ \begin{array}{cc}
     \cos \psi_q^d & \sin \psi_q^d
    \end{array}\right] \left[ \begin{array}{c}
     \cos \psi_k^d \\ \sin \psi_k^d
    \end{array}\right] \cos \Delta^-_d\\
    = & 
    \sum_{d=1}^{2/D} 
     \cos (\psi_q^d - \psi_k^d) \cos (f_d(\xi_m^d - \xi_n^d))\\
\end{align*}
where $\Delta^-_d = f_d ( \xi_m^d - \xi_n^d )$.

For RoPEPool, we can derive the expression as:
 \begin{align*}
    a_{mn} \approx & \sum_{d=1}^{D/2} \Big\{(q_{m,2d-1} k_{n,2d-1} + q_{m,2d} k_{n,2d}) \cos \Delta^-_d \hspace{1mm} + \\ & (q_{m,2d-1} k_{n,2d} - q_{m,2d} k_{n,2d-1}) \sin \Delta^-_d \hspace{1mm} + \\
    &(q_{m,2d-1} k_{n,2d-1} - q_{m,2d} k_{n,2d}) \sin \Delta^+_d \hspace{1mm} + \\ & 
    (q_{m,2d-1} k_{n,2d} + q_{m,2d} k_{n,2d-1}) \cos \Delta^+_d \Big\}\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    = &
    \sum_{d=1}^{D/2} \Big\{ \left[ \begin{array}{cc}
     q_{m, 2d-1} & q_{m, 2d}
    \end{array}\right]
    \left[ \begin{array}{c}
     k_{n, 2d-1} \\ k_{n, 2d}
    \end{array}\right]\cos \Delta^-_d + \\ & 
    \left[ \begin{array}{cc}
     q_{m, 2d-1} & q_{m, 2d}
    \end{array}\right]
    \left[ \begin{array}{c}
     k_{n, 2d} \\ -k_{n, 2d-1}
    \end{array}\right]\sin \Delta^-_d + \\
     & 
    \left[ \begin{array}{cc}
     q_{m, 2d-1} & q_{m, 2d}
    \end{array}\right]
    \left[ \begin{array}{c}
     k_{n, 2d-1} \\ - k_{n, 2d}
    \end{array}\right]\sin \Delta^+_d + \\ & \left[ \begin{array}{cc}
     q_{m, 2d-1} & q_{m, 2d}
    \end{array}\right]
    \left[ \begin{array}{c}
     k_{n, 2d} \\ k_{n, 2d-1}
    \end{array}\right]\cos \Delta^+_d \Big\}\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    = & 
    \sum_{d=1}^{D/2} \left[ \begin{array}{cc}
    \cos \psi_q^d & \sin \psi_q^d
    \end{array}\right]
    \left[ \begin{array}{c}
     \cos \psi_k^d \\ \sin \psi_k^d
    \end{array}\right]\cos \Delta^-_d 
    + \\ & 
    \left[ \begin{array}{cc}
     \cos \psi_q^d & \sin \psi_q^d
    \end{array}\right]
    \left[ \begin{array}{c}
     \sin \psi_k^d \\ -\cos \psi_k^d \\
    \end{array}\right]\sin \Delta^-_d + \\
     & 
    \left[ \begin{array}{cc}
    \cos \psi_q^d & \sin \psi_q^d
    \end{array}\right]
    \left[ \begin{array}{c}
     \cos \psi_k^d \\ - \sin \psi_k^d
    \end{array}\right]\sin \Delta^+_d + \\ & 
    \left[ \begin{array}{cc}
    \cos \psi_q^d & \sin \psi_q^d 
    \end{array}\right]
    \left[ \begin{array}{c}
     \sin \psi_k^d \\ \cos \psi_k^d
    \end{array}\right]\cos \Delta^+_d\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    = &
    \sum_{d=1}^{D/2} \cos (\psi_q^d - \psi_k^d )\cos \Delta^-_d \\ & 
    - 
    \sin (\psi_q^d - \psi_k^d ) \sin \Delta^-_d \\ & 
    + 
    \cos (\psi_q^d + \psi_k^d )\sin \Delta^+_d \\ & 
    + \sin (\psi_q^d + \psi_k^d ) \cos \Delta^+_d\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    = & 
     \sum_{d=1}^{D/2} \cos (\psi_q^d - \psi_k^d + \Delta^-_d ) + \sin (\psi_q^d + \psi_k^d + \Delta^+_d )\\ 
    = & \sum_{d=1}^{D/2} \cos (\psi_q^d - \psi_k^d + f_d(\xi_m^d - \xi_n^d)) \\ & + \sin (\psi_q^d + \psi_k^d + f_d(\xi_m^d + \xi_n^d) )\\
    = & \sum_{d=1}^{D/2} \cos ((\psi_q^d + f_d\xi_m^d) - (\psi_k^d + f_d\xi_n^d)) \\ & + \sin ((\psi_q^d + f_d\xi_m^d) + (\psi_k^d + f_d\xi_n^d))\\
    = & \sum_{d=1}^{D/2} \cos ((\psi_q^d + f_d\xi_m^d) - (\psi_k^d + f_d\xi_n^d)) +\\ &  \cos ((\psi_q^d + f_d\xi_m^d) + (\psi_k^d + f_d\xi_n^d) - \frac{\pi}{2})\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    & [ \text{Use} \cos X + \cos Y = 2 \cos ( \frac{X+Y}{2} ) \cos ( \frac{X-Y}{2} ) ] \\
    % = & \sum_{d=1}^{D/2} 2 \cos \left( \frac{A - B}{2} + \frac{\pi}{4} \right) \cos \left( \frac{A + B}{2} + \frac{\pi}{4} \right)\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    = & \sum_{d=1}^{D/2} 2 \cos \left( \psi_q^d + f_d \xi_m^d - \frac{\pi}{4} \right) \cos \left( \psi_k^d + f_d \xi_n^d - \frac{\pi}{4} \right)
\end{align*}
% where 
% \begin{align*}
% A &= \psi_q^d - \psi_k^d - f_d(\xi_m^d - \xi_n^d) \\
% B &= \psi_q^d + \psi_k^d + f_d(\xi_m^d + \xi_n^d)
% \end{align*}

==> sections/proofs/proof2.tex <==
\noindent\textbf{II. To show that:} F-StrIPE$_1$ has the cross-dimension independence property.\\

\noindent For this, we need to do the following steps:
\begin{enumerate}
    \item Find the complex-valued unpooled feature transform $\mathcal{U}_z(\cdot)$ corresponding to the real-valued unpooled feature transform $\mathcal{U}(\cdot)$, such that $\mathcal{U}(\mathbf{q}_m) \mathcal{U}(\mathbf{k}_n)^\top = \mathfrak{Re} \Big( \mathcal{U}_z(\mathbf{q}_m) \mathcal{U}_z(\mathbf{k}_n)^\top \Big)$ 
    \item Find the complex-valued pooled feature transform $\mathcal{C}_z(\cdot)$ for $\mathcal{U}_z(\cdot)$ and compute the real-valued pooled feature transform $\mathcal{C}(\cdot)$ corresponding to $\mathcal{C}_z(\cdot)$
    \item Show that, since:
    \begin{enumerate}
        \item $\mathcal{U}(\mathbf{q}_m) \mathcal{U}(\mathbf{k}_n)^\top = \mathfrak{Re} \Big( \mathcal{U}_z(\mathbf{q}_m) \mathcal{U}_z(\mathbf{k}_n)^\top \Big)$
        \item $\mathcal{U}_z(\mathbf{q}_m) \mathcal{U}_z(\mathbf{k}_n)^\top = \mathcal{C}_z(\mathbf{q}_m) \mathcal{C}_z(\mathbf{k}_n)^\top$
        \item $\mathcal{C}(\mathbf{q}_m) \mathcal{C}(\mathbf{k}_n)^\top = \mathfrak{Re} \Big( \mathcal{C}_z(\mathbf{q}_m) \mathcal{C}_z(\mathbf{k}_n)^\top \Big)$
    \end{enumerate}
    we have that $\mathcal{U}(\mathbf{q}_m) \mathcal{U}(\mathbf{k}_n)^\top = \mathcal{C}(\mathbf{q}_m) \mathcal{C}(\mathbf{k}_n)^\top$, as desired.
\end{enumerate}

For step 1, we can use equations (17) and (20) from the paper to get the unpooled feature map for F-StrIPE$_1$:
\begin{equation}
    \mathcal{U}(\mathbf{a}_t) : \mathbf{a}_t \mapsto  
    \begin{bmatrix} 
    a_{1} \cos (2 \pi f_1 p_t) \\ 
    a_{1} \sin (2 \pi f_1 p_t) \\ 
    \vdots \\ 
    a_{D} \cos (2 \pi f_D p_t) \\ 
    a_{D} \sin (2 \pi f_D p_t) 
    \end{bmatrix}^\top
\end{equation}
We can calculate the complex-valued unpooled feature map by noting that:
\begin{align}
    \mathcal{U}(\mathbf{q}_m) \mathcal{U}(\mathbf{k}_n)^\top &= \sum_{d=1}^D q_{dm} k_{dn} \cos ( 2 \pi f_{d} ( p_m - p_n ) ) \\
    &= \mathfrak{Re} \big( \sum_{d=1}^D q_{dm} k_{dn} \exp ( 2\pi i f_{d} ( p_m - p_n ) ) \big)
\end{align}
Then, we can derive the complex-valued feature map by expanding the complex-valued sum above as:
% \begin{align}
%     \mathcal{U}_z(\mathbf{a}_t) : \mathbf{a}_t &\mapsto  
%     \begin{bmatrix} 
%     q_{1m} \exp (2 \pi i f_1 p_t) \\ 
%     \vdots \\ 
%     q_{Dm} \exp (2 \pi i f_D p_t) 
%     \end{bmatrix}^\top \\
%     \mathcal{U}_z(\mathbf{k}_n) : \mathbf{k}_n &\mapsto  
%     \begin{bmatrix} 
%     k_{1n} \exp (- 2 \pi i f_1 p_n) \\ 
%     \vdots \\ 
%     k_{Dn} \exp (- 2 \pi i f_D p_n) 
%     \end{bmatrix}^\top
% \end{align}
\begin{equation}
    \mathcal{U}_z(\mathbf{a}_t) : \mathbf{a}_t \mapsto  
    \begin{bmatrix} 
    a_{1t} \exp (2 \pi i f_1 p_t) \\ 
    \vdots \\ 
    a_{Dt} \exp (2 \pi i f_D p_t) 
    \end{bmatrix}^\top
\end{equation}
with the feature transform for queries being $\mathcal{U}_z(\mathbf{q}_m)$ and for keys being $\mathcal{U}^{\dagger}_z(\mathbf{k}_n)$, where $\dagger$ denotes that we take the complex conjugate of $\mathcal{U}_z(\mathbf{k}_n)$ elementwise.
Note that this exactly matches the expected expression for stationary, positive-definite kernels~\cite{rahimi_random_2007}. Clearly, $\mathcal{U}(\mathbf{q}_m) \mathcal{U}(\mathbf{k}_n)^\top = \mathfrak{Re} \Big( \mathcal{U}_z(\mathbf{q}_m) \mathcal{U}_z^\dagger(\mathbf{k}_n)^\top \Big)$.

For step 2, we can find the complex-valued pooled feature transforms for keys and queries by adding up the dimensions of the unpooled complex-valued transform.
% \begin{align}
%     \mathcal{C}_z(\mathbf{q}_m) : \mathbf{q}_m &\mapsto \left[ \sum_{d=1}^D q_{dm} \exp (2 \pi i f_d p_m) \right]^\top \label{eq:complex_feature1} \\
%     \mathcal{C}_z(\mathbf{k}_n) : \mathbf{k}_n &\mapsto \left[ \sum_{d=1}^D k_{dn} \exp (- 2 \pi i f_d p_n) \right]^\top \label{eq:complex_feature2}
% \end{align}
\begin{equation}
    \mathcal{C}_z(\mathbf{a}_t) : \mathbf{a}_t \mapsto \left[ \sum_{d=1}^D a_{dt} \exp (2 \pi i f_d p_t) \right]^\top \label{eq:complex_feature1}
\end{equation}
with the pooled transform for queries being $\mathcal{C}_z (\mathbf{q}_m)$ and for keys being $\mathcal{C}_z^\dagger (\mathbf{k}_n)$.
To write down the real-valued pooled feature transform $\mathcal{C}(\cdot)$, we first write down $ \mathfrak{Re} \big( \mathcal{C}_z(\mathbf{q}_m) \mathcal{C}_z^\dagger(\mathbf{k}_n)^\top \big)$, which is as follows:
\begin{align}
    \mathcal{C}_z(\mathbf{q}_m) : \mathbf{q}_m &\mapsto \left[ \sum_{d=1}^D q_{dm} \big( \cos (2 \pi f_d p_m) + i \sin (2 \pi f_d p_m) \big) \right]^\top \\
    \mathcal{C}_z^\dagger(\mathbf{k}_n) : \mathbf{k}_n &\mapsto \left[ \sum_{d=1}^D k_{dn} \big( \cos (2 \pi f_d p_n) - i \sin (2 \pi f_d p_n) \big) \right]^\top
\end{align}
\begin{equation}
    \begin{split}
    \mathfrak{Re} \big( \mathcal{C}_z(\mathbf{q}_m) \mathcal{C}_z^\dagger(\mathbf{k}_n)^\top \big) = 
    \big( \sum_{d=1}^D &q_{dm} \big( \cos (2 \pi f_d p_m) \big) \\ 
    &\big( \sum_{d^\prime=1}^D k_{d^\prime n} \big( \cos (2 \pi f_{d^\prime} p_n) \big) + \\
    \big( \sum_{d=1}^D &q_{dm} \big( \sin (2 \pi f_d p_m) \big) \\ 
    &\big( \sum_{d^\prime=1}^D k_{d^\prime n} \big( \sin (2 \pi f_{d^\prime} p_n) \big)
    \end{split}
\end{equation}
We can turn this expression into a matrix multiplication form to get:
\begin{equation}
    \mathcal{C}(\mathbf{a}_t) : \mathbf{a}_t \mapsto
    \begin{bmatrix} 
    \sum_{d=1}^D a_d \cos (2 \pi f_d p_t) \\ 
    \sum_{d=1}^D a_d \sin (2 \pi f_d p_t)
    \end{bmatrix}^\top
\end{equation}
Again, by design, we obtain that $\mathcal{C}(\mathbf{q}_m) \mathcal{C}(\mathbf{k}_n)^\top = \mathfrak{Re} \Big( \mathcal{C}_z(\mathbf{q}_m) \mathcal{C}_z^\dagger(\mathbf{k}_n)^\top \Big)$

For step 3, we need to only prove that substeps a, b, and c are true. We already proved 3a and 3c in steps 1 and 2, respectively, above. For 3b, we use a basic fact from harmonic analysis, namely, that complex exponentials with different frequencies are orthogonal, and thus, when we calculate $\mathcal{C}_z(\mathbf{q}_m) \mathcal{C}_z^\dagger(\mathbf{k}_n)^\top$ using equation (\ref{eq:complex_feature1}), the multiplications of the cross-dimension terms terms evaluate to 0. This completes the proof for step 3b. \qed \\


% For  F-StrIPE$_1$, given the \textit{pooled feature map} $\mathcal{U}(\cdot)$ (corresponding to Equations \ref{eq:unpooled_fstripe1_1}-\ref{eq:unpooled_fstripe1_2} in the main paper):
% \begin{equation*}
%     \mathcal{U}(\mathbf{a}_i) : \mathbf{a}_i \mapsto  
%     \begin{bmatrix} 
%     a_{1} \cos (2 \pi f_1 p_i) \\ 
%     a_{1} \sin (2 \pi f_1 p_i) \\ 
%     \vdots \\ 
%     a_{D} \cos (2 \pi f_D p_i) \\ 
%     a_{D} \sin (2 \pi f_D p_i) 
%     \end{bmatrix}^\top
% \end{equation*}
% and the \textit{pooled feature map} $\mathcal{C}(\cdot)$ (corresponding to Equations \ref{eq:pooled_fstripe1_1}-\ref{eq:pooled_fstripe1_2} in the main paper):
% \begin{equation*}
%     \mathcal{C}(\mathbf{a}_i) : \mathbf{a}_i \mapsto
%     \begin{bmatrix} 
%     \sum_{d=1}^D a_d \cos (2 \pi f_d p_i) \\ 
%     \sum_{d=1}^D a_d \sin (2 \pi f_d p_i)
%     \end{bmatrix}^\top
% \end{equation*}
% show that $\mathcal{U}(\mathbf{q}_m) \mathcal{U}(\mathbf{k}_n)^\top = \mathcal{C}(\mathbf{q}_m) \mathcal{C}(\mathbf{k}_n)^\top$. \\

% \noindent To do this, we need to use the fact that $\mathcal{U}(\cdot)$ originates from kernel approximation theory, which relies on definitions of kernels in the complex domain. We can obtain the complex-valued unpooled feature map by first observing that, by using the real-valued unpooled feature map, we can write:
% \begin{align}
%     \mathcal{U}(\mathbf{q}_m) \mathcal{U}(\mathbf{k}_n)^\top &= \sum_{d=1}^D q_{dm} k_{dn} \cos ( 2 \pi f_{d} ( p_m - p_n ) ) \\
%     &= \sum_{d=1}^D q_{dm} k_{dn} \exp ( 2\pi i f_{d} ( p_m - p_n ) )
% \end{align}
% Thus, $\mathcal{U}^i(\cdot)$, the complex version of the unpooled feature map, is as follows for queries and keys:
% \begin{align}
%     \mathcal{U}^i(\mathbf{q}_m) : \mathbf{q}_m &\mapsto  
%     \begin{bmatrix} 
%     q_{1m} \exp (2 \pi i f_1 p_m) \\ 
%     \vdots \\ 
%     q_{Dm} \exp (2 \pi i f_D p_m) 
%     \end{bmatrix}^\top \\
%     \mathcal{U}^i(\mathbf{k}_n) : \mathbf{k}_n &\mapsto  
%     \begin{bmatrix} 
%     k_{1n} \exp (- 2 \pi i f_1 p_n) \\ 
%     \vdots \\ 
%     k_{Dn} \exp (- 2 \pi i f_D p_n) 
%     \end{bmatrix}^\top
% \end{align}
% Clearly, $\mathcal{U}(\mathbf{q}_m) \mathcal{U}(\mathbf{k}_n)^\top = \mathcal{U}^i(\mathbf{q}_m) \mathcal{U}^i(\mathbf{k}_n)^\top$. By adding up the dimensions in $\mathcal{U}^i(\cdot)$, the pooled versions of $\mathcal{U}^i(\cdot)$ for queries and keys can written as:
% \begin{align}
%     \mathcal{C}^i(\mathbf{q}_m) : \mathbf{q}_m &\mapsto \left[ \sum_{d=1}^D q_{dm} \exp (2 \pi i f_d p_m) \right]^\top \\
%     \mathcal{C}^i(\mathbf{k}_n) : \mathbf{k}_n &\mapsto \left[ \sum_{d=1}^D k_{dn} \exp (- 2 \pi i f_d p_n) \right]^\top
% \end{align}
% Then, we can use the following fact:
% \begin{equation} \label{eq:orth_bases}
%     \exp (2 \pi i f_p t) \cdot \exp (2 \pi i f_q t) 
%     \begin{cases}
%         1, &\text{ if } f_p = f_q \\
%         0, &\text{ otherwise }
%     \end{cases}
% \end{equation}
% to obtain $\mathcal{U}^i(\mathbf{q}_m) \mathcal{U}^i(\mathbf{k}_n)^\top = \mathcal{C}^i(\mathbf{q}_m) \mathcal{C}^i(\mathbf{k}_n)^\top$. The only thing left to do is to find the real-valued pooled feature map corresponding to $\mathcal{C}^i(\cdot)$ and show that this is equivalent to $\mathcal{C}(\cdot)$. For this, we can simply write:
% \begin{align}
%     \mathcal{C}^i(\mathbf{q}_m) : \mathbf{q}_m &\mapsto \left[ \sum_{d=1}^D q_{dm} \big( \cos (2 \pi f_d p_m) + i \sin (2 \pi f_d p_m) \big) \right]^\top \\
%     \mathcal{C}^i(\mathbf{k}_n) : \mathbf{k}_n &\mapsto \left[ \sum_{d=1}^D k_{dn} \big( \cos (2 \pi f_d p_n) - i \sin (2 \pi f_d p_n) \big) \right]^\top
% \end{align}
% Then, we can write the product $\mathcal{C}^i(\mathbf{q}_m) \mathcal{C}^i(\mathbf{k}_n)^\top$ as:
% \begin{equation}
%     \begin{split}
%     \mathcal{C}^i(\mathbf{q}_m) \mathcal{C}^i(\mathbf{k}_n)^\top = 
%     \big( \sum_{d=1}^D &q_{dm} \big( \cos (2 \pi f_d p_m) \big) \\ 
%     &\big( \sum_{d^\prime=1}^D k_{d^\prime n} \big( \cos (2 \pi f_{d^\prime} p_n) \big) + \\
%     \big( \sum_{d=1}^D &q_{dm} \big( \sin (2 \pi f_d p_m) \big) \\ 
%     &\big( \sum_{d^\prime=1}^D k_{d^\prime n} \big( \sin (2 \pi f_{d^\prime} p_n) \big)
%     \end{split}
% \end{equation}
% Here, we can exclude the products that contain the imaginary unit $i$ because the family of kernels we are considering are real-valued. This gives us the desired pooled feature map of Equations \ref{eq:pooled_fstripe1_1}-\ref{eq:pooled_fstripe1_2} in the real domain. 

% In summary, by showing that $\mathcal{U}^i(\mathbf{q}_m) \mathcal{U}^i(\mathbf{k}_n)^\top = \mathcal{C}^i(\mathbf{q}_m) \mathcal{C}^i(\mathbf{k}_n)^\top$ in the complex domain, and showing that the real-valued feature maps corresponding to $\mathcal{U}^i(\mathbf{a}_i)$ and $\mathcal{C}^i(\mathbf{a}_i)$ are $\mathcal{U}(\mathbf{a}_i)$ and $\mathcal{C}(\mathbf{a}_i)$ respectively, we proved that $\mathcal{U}(\mathbf{q}_m) \mathcal{U}(\mathbf{k}_n)^\top = \mathcal{C}(\mathbf{q}_m) \mathcal{C}(\mathbf{k}_n)^\top$. Note that we only demonstrated this property for F-StrIPE$_1$ but the proof can be easily extended to the case of F-StrIPE with $N_f > 1$. \qed \\

==> sections/proofs/proof_ropepool.tex <==
\noindent\textbf{III. Derivation for RoPEPool} corresponding to Equation (23).\\

\noindent Similar to the proof above, we will find $\mathcal{U}(\cdot)$, $\mathcal{C}(\cdot)$, $\mathcal{U}_z(\cdot)$ and $\mathcal{C}_z(\cdot)$ for RoPE. As shown in Fig. \ref{fig:drawing} below, we are interested in the expression $\mathcal{C}(\mathbf{q}_m) \mathcal{C}(\mathbf{k}_n)^\top$, since this will give us the real-valued expression for RoPEPool, as desired in Equation (23).

\begin{figure}[b]
    \centering
    \includegraphics[width=1.75in]{figs/drawing.png}
    \caption{RoPE vs RoPEPool}
    \label{fig:drawing}
\end{figure}

From equations (21) and (22) in the paper, we can find the complex-valued counterpart $\mathcal{U}_z(\cdot)$ for $\mathcal{U}(\cdot)$ by using:
\begin{align}
    % \cos x &= \frac{\exp^{ix}}{2} + \frac{\exp^{-ix}}{2} \\
    % \sin x &= i \frac{\exp^{-ix}}{2} - i \frac{\exp^{ix}}{2}
    \cos x &= \frac{\exp^{ix} + \exp^{-ix}}{2} \\
    \sin x &= \frac{\exp^{-ix} - \exp^{ix}}{2\ch{i}}
\end{align}
Then, we have:
\begin{equation}
    \mathcal{U}_z(\mathbf{a}_i) : \mathbf{a}_i \mapsto  
    \frac{1}{2}\begin{bmatrix} 
    \substack{
        \big( a_{1} e(+,1,i) + a_{1} e(-,1,i) \\ - a_{2} i e(-,1,i) + a_{2} i e(+,1,i) \big)
    } \\ 
    \substack{
        \big( a_{2} e(+,1,i) + a_{2} e(-,1,i) \\ + a_{1} i e(-,1,i) - a_{1} i e(+,1,i) \big)
    } \\ 
    \vdots \\ 
    \substack{
        \big( a_{D-1} e(+,D/2,i) + a_{D-1} e(-,D/2,i) \\ - a_{D} i e(-,D/2,i) + a_{D} i e(+,D/2,i) \big)
    } \\ 
    \substack{
        \big( a_{D} e(+,D/2,i) + a_{D} e(-,D/2,i) \\ + a_{D-1} i e(-,D/2,i) - a_{D-1} i e(+,D/2,i) \big)
    } \\ 
    \end{bmatrix}^\top
\end{equation}
where we used the function $e(+,j,k) = \exp^{2 \pi i f_j p_k}$ and $e(-,j,k) = \exp^{-2 \pi i f_j p_k}$.

The complex-valued pooled feature transform $\mathcal{C}_z(\mathbf{a}_i)$ corresponding to $\mathcal{U}_z(\mathbf{a}_i)$ can be obtained by adding up all the dimensions in $\mathcal{U}_z(\mathbf{a}_i)$:
\begin{equation}
    \mathcal{C}_z(\mathbf{a}_i) : \mathbf{a}_i \mapsto
    \frac{1}{2}\begin{bmatrix} 
    \sum_{d=1}^{D/2}
    \substack{
    \big( a_{2d-1} (1-i) + a_{2d} (1+i) \big) \exp^{2 \pi i f_d p_i}\\+ \big( a_{2d-1} (1+i) + a_{2d} (1-i) \big) \exp^{-2 \pi i f_d p_i}
    }
    \end{bmatrix}^\top
\end{equation}
Then, $\mathcal{C}_z(\mathbf{q}_m) \mathcal{C}_z(\mathbf{k}_n)^\top$ can be calculated as:
\begin{align*}
    \mathcal{C}_z(\mathbf{q}_m) &\mathcal{C}_z(\mathbf{k}_n)^\top = \\ & \Bigg[ \frac{1}{2} \sum_{d=1}^{D/2} \Big\{ \big( q_{2d-1} (1-i) + q_{2d} (1+i) \big) \exp^{2 \pi i f_d p_m} + \\ &\big( q_{2d-1} (1+i) + q_{2d} (1-i) \big) \exp^{-2 \pi i f_d p_m} \Big\} \Bigg] \cdot \\ &\Bigg[\frac{1}{2}\sum_{d=1}^{D/2}\Big\{ \big( k_{2d-1} (1-i) + k_{2d} (1+i) \big) \exp^{2 \pi i f_d p_n} + \\ &\big( k_{2d-1} (1+i) + k_{2d} (1-i) \big) \exp^{-2 \pi i f_d p_n} \Big\}\Bigg]
\end{align*}
Resolving this product will lead to a sum of four terms. We can again use the orthogonality of complex exponentials to obtain:
\begin{align*}
    \mathcal{C}_z&(\mathbf{q}_m) \mathcal{C}_z(\mathbf{k}_n)^\top = \frac{1}{4} \sum_{d=1}^{D/2} \\
    &\big( q_{2d-1} (1-i) + q_{2d} (1+i) \big) \\&\big( k_{2d-1} (1-i) + k_{2d} (1+i) \big) \exp^{2 \pi i f_d (p_m+p_n)} + \\
    &\big( q_{2d-1} (1-i) + q_{2d} (1+i) \big) \\&\big( k_{2d-1} (1+i) + k_{2d} (1-i) \big) \exp^{2 \pi i f_d (p_m-p_n)} + \\
    &\big( q_{2d-1} (1+i) + q_{2d} (1-i) \big) \\&\big( k_{2d-1} (1-i) + k_{2d} (1+i) \big) \exp^{-2 \pi i f_d (p_m-p_n)} + \\
    &\big( q_{2d-1} (1+i) + q_{2d} (1-i) \big) \\&\big( k_{2d-1} (1+i) + k_{2d} (1-i) \big) \exp^{-2 \pi i f_d (p_m+p_n)}
\end{align*}
We can use the following to simplify each of the four terms:
\begin{align*}
    (1 + i)^2 &= 2i \\
    (1 - i)^2 &= -2i \\
    (1 + i)(1-i) &= 2 \\
\end{align*}
and we obtain:
\begin{align*}
    \mathcal{C}_z(\mathbf{q}_m) \mathcal{C}_z&(\mathbf{k}_n)^\top = \frac{1}{2} \sum_{d=1}^{D/2} \\
    &\big( - i q_{2d-1} k_{2d-1} + q_{2d-1} k_{2d} +  q_{2d} k_{2d-1} + i q_{2d} k_{2d} \big)\\&\exp^{2 \pi i f_d (p_m+p_n)} + \\
    &\big( q_{2d-1} k_{2d-1} - i q_{2d-1} k_{2d} + i q_{2d} k_{2d-1} + q_{2d} k_{2d} \big)\\&\exp^{2 \pi i f_d (p_m-p_n)} + \\
    &\big( q_{2d-1} k_{2d-1} + i q_{2d-1} k_{2d} - i q_{2d} k_{2d-1} + q_{2d} k_{2d} \big)\\&\exp^{-2 \pi i f_d (p_m-p_n)} + \\
    &\big( i q_{2d-1} k_{2d-1} + q_{2d-1} k_{2d} + q_{2d} k_{2d-1} - i q_{2d} k_{2d} \big)\\&\exp^{-2 \pi i f_d (p_m+p_n)} \numberthis \label{eq:rope_pooled_attn_imaginary}
\end{align*}
The real-valued counterpart of this is $\mathfrak{Re} \big( \mathcal{C}_z(\mathbf{q}_m) \mathcal{C}_z(\mathbf{k}_n)^\top \big) = \mathcal{C}(\mathbf{q}_m) \mathcal{C}(\mathbf{k}_n)^\top$, which is:
\begin{align*}
    \mathcal{C}(\mathbf{q}_m) \mathcal{C}&(\mathbf{k}_n)^\top = \sum_{d=1}^{D/2} \Big\{ \\ 
    &(q_{m,2d-1} k_{n,2d-1} + q_{m,2d} k_{n,2d}) \cos \big( 2 \pi f_d (p_m - p_n) \big) + \\
    &(q_{m,2d-1} k_{n,2d} - q_{m,2d} k_{n,2d-1}) \sin \big( 2 \pi f_d (p_m - p_n) \big) + \\
    &(q_{m,2d-1} k_{n,2d-1} - q_{m,2d} k_{n,2d}) \sin \big( 2 \pi f_d (p_m + p_n) \big) + \\
    &(q_{m,2d-1} k_{n,2d} + q_{m,2d} k_{n,2d-1}) \cos \big( 2 \pi f_d (p_m + p_n) \big) \Big\}
\end{align*}

Note that, we do not prove this here, but we can show that $\mathcal{U}(\mathbf{q}_m) \mathcal{U}(\mathbf{k}_n)^\top \neq \mathcal{C}(\mathbf{q}_m) \mathcal{C}(\mathbf{k}_n)^\top$, which is precisely the fact that RoPE lacks the cross-dimension independent property (also illustrated in Fig. \ref{fig:drawing}). \qed \\

==> sections/proofs/sketch_prop1.tex <==
\noindent\textbf{I. Proof sketch for Proposition 1}, which states that Equation (4) defines attention as a Tensor Product Kernel:
\begin{equation}
    a_{mn}^d = \kappa(q_{md}, k_{nd}) \times \chi_d (p_m, p_n)
\end{equation}\\

\noindent The first step is to notice that the following holds $\forall d \in \{ 1, ..., D \}$:
\begin{equation} \label{eq:sketch_prop1}
    \mathbf{A}_d = \text{diag}(\mathbf{Q}_{:,d}) \mathbf{P}_d \text{diag}(\mathbf{K}_{:,d}) = \mathbf{Q}_{:,d} \mathbf{K}_{:,d}^\top \odot \mathbf{P}_d
\end{equation}
where $\odot$ is the Hadamard product. Then, 
\begin{align}
    a_{mn} &= \left[ \sum_{d=1}^D \text{diag}(\mathbf{Q}_{:,d}) \mathbf{P}_d \text{diag}(\mathbf{K}_{:,d}) \right]_{mn} \\
    &= \left[ \sum_{d=1}^D \mathbf{A}_d \right]_{mn} \\
    &= \sum_{d=1}^D a_{mn}^d \numberthis \label{eq:sketch_prop2}
\end{align}
Then, from Equation \ref{eq:sketch_prop1}, we can write:
\begin{equation} \label{eq:sketch_prop3}
    a_{mn}^d = \kappa(q_{md}, k_{nd}) \times \chi_d (p_m, p_n)
\end{equation}
where $\kappa(q_{md}, k_{nd}) = q_{md} k_{nd}$ and $\chi_d (p_m, p_n) = \left[ \mathbf{P}_d \right]_{mn}$. \qed \\

==> sections/results_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\resizebox{2.05\columnwidth}{!}{%
\begin{tabular}{cc|cccc|cccc}
\hline
\multirow{3}{*}{\textbf{Method}} & \multirow{3}{*}{\textbf{Information}} & \multicolumn{4}{c|}{\textbf{Train = 16 bars; Test = 16 bars}} & \multicolumn{4}{c}{\textbf{Train = 16 bars; Test = 16 bars}} \\
 &  & \textbf{CS} & \textbf{SSMD} & \textbf{GS} & \textbf{NDD} & \textbf{CS} & \textbf{SSMD} & \textbf{GS} & \textbf{NDD} \\
 &  & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ \\ \hline \hline
\textbf{RoPE} & \multirow{3}{*}{Time} & 2.61 ± 0.16 & 29.31 ± 0.0 & 7.6 ± 0.15 & 103.31 ± 0.04 & 2.22 ± 0.02 & 27.61 ± 0.0 & 8.47 ± 0.03 & 102.74 ± 0.03 \\
\textbf{F-StrIPE$_1$} &  & 5.16 ± 2.89 & 29.29 ± 0.04 & 11.02 ± 3.5 & 102.9 ± 0.67 & 6.92 ± 1.27 & 27.59 ± 0.0 & 20.98 ± 2.79 & 101.66 ± 0.17 \\
\textbf{RoPEPool} &  & 3.4 ± 3.09 & 29.31 ± 0.03 & 8.92 ± 3.9 & 103.31 ± 0.67 & 7.15 ± 0.76 & 27.57 ± 0.01 & 21.69 ± 1.99 & 101.52 ± 0.12 \\ \hline \hline
\textbf{RoPE} & \multirow{3}{*}{RNT} & 17.6 ± 0.61 & 28.76 ± 0.04 & 24.38 ± 0.92 & 97.17 ± 0.22 & 17.31 ± 1.45 & 26.93 ± 0.04 & 48.0 ± 2.14 & 95.12 ± 0.28 \\
\textbf{F-StrIPE$_1$} &  & 17.67 ± 1.15 & 28.76 ± 0.06 & 24.74 ± 1.39 & 97.55 ± 0.56 & 13.38 ± 1.29 & 27.17 ± 0.08 & 37.17 ± 2.25 & 97.65 ± 0.53 \\
\textbf{RoPEPool} &  & 13.89 ± 1.34 & 28.92 ± 0.04 & 20.28 ± 2.2 & 98.98 ± 0.29 & 11.21 ± 0.15 & 27.39 ± 0.02 & 33.62 ± 0.9 & 98.89 ± 0.43 \\ \hline
\textbf{RoPE} & \multirow{3}{*}{KMT} & 10.11 ± 5.26 & 29.06 ± 0.15 & 16.41 ± 6.31 & 100.64 ± 1.77 & 15.6 ± 2.69 & 27.25 ± 0.01 & 42.74 ± 4.87 & 97.24 ± 0.4 \\
\textbf{F-StrIPE$_1$} &  & 19.72 ± 0.38 & 28.21 ± 0.03 & 24.18 ± 0.48 & 92.97 ± 0.17 & 23.34 ± 0.51 & 26.44 ± 0.06 & 60.18 ± 1.23 & 90.39 ± 0.19 \\
\textbf{RoPEPool} &  & 21.55 ± 2.41 & 28.43 ± 0.12 & 27.09 ± 3.59 & 94.38 ± 0.46 & 22.28 ± 1.28 & 26.64 ± 0.11 & 58.69 ± 2.56 & 91.7 ± 0.84 \\ \hline
\textbf{RoPE} & \multirow{3}{*}{BIN} & 1.77 ± 0.09 & 29.32 ± 0.0 & 6.93 ± 0.1 & 103.57 ± 0.02 & 4.31 ± 3.05 & 27.6 ± 0.0 & 14.14 ± 8.51 & 102.18 ± 0.75 \\
\textbf{F-StrIPE$_1$} &  & 24.98 ± 0.31 & \textbf{27.44 ± 0.06} & 28.18 ± 0.3 & \textbf{89.42 ± 0.32} & \textbf{28.3 ± 0.51} & \textbf{25.86 ± 0.09} & 71.36 ± 0.44 & \textbf{87.35 ± 0.46} \\
\textbf{RoPEPool} &  & \textbf{25.2 ± 0.53} & 27.57 ± 0.09 & \textbf{28.52 ± 0.46} & 89.65 ± 0.37 & 28.05 ± 0.4 & 26.06 ± 0.08 & \textbf{71.54 ± 0.85} & 87.95 ± 0.34 \\ \hline
\end{tabular}%
}
\caption{Results table}
\label{tab:results}
\end{table*}
